Non-empirical prediction of the length-dependent ionization potential in molecular chains

The ionization potential of molecular chains is well-known to be a tunable nano-scale property that exhibits clear quantum confinement effects. State-of-the-art methods can accurately predict the ionization potential in the small molecule limit and in the solid-state limit, but for intermediate, nano-sized systems prediction of the evolution of the electronic structure between the two limits is more difficult. Recently, optimal tuning of range-separated hybrid functionals has emerged as a highly accurate method for predicting ionization potentials. This was first achieved for molecules using the ionization potential theorem (IPT) and more recently extended to solid-state systems, based on an \textit{ansatz} that generalizes the IPT to the removal of charge from a localized Wannier function. Here, we study one-dimensional molecular chains of increasing size, from the monomer limit to the infinite polymer limit using this approach. By comparing our results with other localization-based methods and where available with experiment, we demonstrate that Wannier-localization-based optimal tuning is highly accurate in predicting ionization potentials for any chain length, including the nano-scale regime.

==> backup.tex <==
The reasons for the failure of standard DFT in predicting these quantities lies fundamentally within the theory and is already well-established. The most common approach used in DFT calculations is the Kohn-Sham (KS) approach \cite{kohn_sham_1965}, which is exact in principle but in practice requires an approximation to the unknown exchange-correlation energy as a functional of the electron density \cite{KochW.&Holthausen2001, kuemmel_kronik_2008}. The exact KS total energy is piecewise linear as a function of the fractional particle number. Upon applying Janak's theorem, one obtains the ionization potential theorem (IPT) according to which $\textrm{IP}=-\epsilon_H$, where $\epsilon_H$ is the highest occupied KS orbital eigenvalue. On the other hand, the lowest unoccupied KS orbital eigenvalue in the same KS spectrum, $\epsilon_L$, is different from the EA. This is because the exact KS total energy features a derivative discontinuity (DD), $\Delta_{\textrm{xc}}$, in the exchange-correlation energy upon crossing an integer number of particles. This DD propagates into the eigenvalue spectrum such that $\textrm{EA} = - \epsilon_L - \Delta_{\textrm{xc}}$, and accordingly $E_g = \epsilon_L - \epsilon_H + \Delta_{\textrm{xc}}$. This implies that even in principle, the KS approach is unable of providing the correct fundamental gap. Indeed, fundamental gaps are typically severely underestimated when using standard KS approximations. In virtue of the IPT, the IP itself can be obtained accurately from the exact KS highest occupied eigenvalue. In practice, upon using approximate functionals, this is no longer the case. All approximate KS functionals have a missing DD, which goes hand in hand with deviation from piecewise linearity, and the IPT breaks.
